Sudakov Shoulder Resummation for Thrust and Heavy Jet Mass

When the allowed range of an observable grows order-by-order in perturbation theory, its perturbative expansion can have discontinuities (as in the $C$ parameter) or discontinuities in its derivatives (as in thrust or heavy jet mass) called Sudakov shoulders. We explore the origin of these logarithms using both perturbation theory and effective field theory. We show that for thrust and heavy jet mass, the logarithms arise from kinematic configurations with narrow jets and deduce the next-to-leading logarithmic series. The left-shoulder logarithms in heavy jet mass ($\rho$) of the form $r\ \alpha_s^n \ln^{2n}r $ with $r=\frac{1}{3}-\rho$ are particularly dangerous, because they invalidate fixed order perturbation theory in regions traditionally used to extract $\alpha_s$. Although the factorization formula shows there are no non-global logarithms, we find Landau-pole like singularities in the resummed distribution associated with the cusp anomalous dimension, and that power corrections are exceptionally important.

==> Sudakov Shoulders/tikzfeynman.keys.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% TikZ-Feynman
% Feynman Diagrams with TikZ
% Copyright (C) 2015  Joshua Ellis
%
%
% This work may be distributed and/or modified under the terms of the GNU General
% Public License as published by the Free Software Foundation, either version 3 
% of the License, or (at your option) any later version.
%
% This program is distributed in the hope that it will be useful, but WITHOUT
% ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or FITNESS
% FOR A PARTICULAR PURPOSE.  See the LaTeX Project Public License for more
% details.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Shapes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Crossed Circle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclareshape{crossed circle}
{
  \inheritsavedanchors[from=circle]
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}

  \inheritbackgroundpath[from=circle]

  \foregroundpath{
    % Compute south west
    \centerpoint
    \pgf@xc=\radius
    \advance\pgf@x by-0.707107\pgf@xc
    \advance\pgf@y by-0.707107\pgf@xc
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y  % Store coordinates
    % Compute north east point
    \centerpoint
    \pgf@xc=\radius
    \advance\pgf@x by0.707107\pgf@xc
    \advance\pgf@y by0.707107\pgf@xc
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y  % Store coordinates
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
    \pgfsetarrowsstart{}
    \pgfsetarrowsend{}
 }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Decorations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Complete Sines
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Complete sines replaces the path with a whole number of sine waves.
%% Thanks to http://tex.stackexchange.com/a/134516/26980
\pgfdeclaredecoration{complete sines}{initial}
{
  %% Begin by computing the overall path length and find how many sine waves we
  %% can fit in.  Nothing happens beyond the computation.
  \state{initial}[
    width=+0pt,
    next state=move,
    persistent precomputation={
      \def\tikzfeynman@cs@angle@step{30}
      \def\tikzfeynman@cs@current@angle{0}
      \pgfmathsetlengthmacro{\tikzfeynman@cs@points@per@step}{
        \pgfdecoratedinputsegmentlength
        / int(\pgfdecoratedinputsegmentlength
        / \pgfdecorationsegmentlength)
        / 360
        * \tikzfeynman@cs@angle@step}
    },
  ]{}
  %% Move to the origin to the path
  \state{move}[
    width=+\tikzfeynman@cs@points@per@step,
    next state=draw
  ]{
    \pgfpathmoveto{\pgfpointorigin}
  }
  %% Draw the sine wave itself.  This computes the value every 20 degrees and draws straight edges.
  \state{draw}[
    width=+\tikzfeynman@cs@points@per@step,
    switch if less than=1.25*\tikzfeynman@cs@points@per@step to final, % <- bit of a hack
    persistent postcomputation={
      \pgfmathparse{mod(\tikzfeynman@cs@current@angle+\tikzfeynman@cs@angle@step, 360)}
      \let\tikzfeynman@cs@current@angle=\pgfmathresult%
    },
  ]{
    \pgfmathparse{sin(\tikzfeynman@cs@current@angle) * \pgfmetadecorationsegmentamplitude / 2}
    \tikz@decoratepathfalse
    \pgfpathlineto{\pgfqpoint{0pt}{\pgfmathresult pt}}%
  }

  \state{final}{
    \ifdim\pgfdecoratedremainingdistance>0pt\relax
      \pgfpathlineto{\pgfpointdecoratedpathlast}
    \fi
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Keys
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzfeynmanset{
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Hooks
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  execute at begin feynman/.code={},
  execute at end feynman/.code={},
  every feynman/.style={/tikzfeynman/every feynman@@/.append style={#1}},
  every feynman@@/.style={
    /tikzfeynman/.cd,
    /tikzfeynman/medium,
  },
  execute at begin feynman@@/.code={}                     %% Internal version
  execute at end feynman@@/.code={},                      %% Internal version
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Diagrams
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every diagram/.style={/tikzfeynman/every diagram@@/.append style={#1}},
  every diagram@@/.style={
    /tikzfeynman/.cd,
    .search also={/tikz/graphs, /tikz},
    nodes={
      /tikzfeynman/.cd,
      /tikzfeynman/.search also={/tikz/graphs, /tikz},
      /tikzfeynman/every vertex@@,
      /tikzfeynman/every vertex},
    edges={
      /tikzfeynman/.cd,
      /tikzfeynman/.search also={/tikz/graphs, /tikz},
      /tikzfeynman/every edge@@,
      /tikzfeynman/every edge},
    /tikzfeynman/medium,
  },
  every inline/.style={/tikzfeynman/inline@@/.append style={#1}},
  every inline@@/.style={
    /tikzfeynman/small,
  },
  inline/.style={
    /tikz/baseline={#1},
    /tikzfeynman/every inline@@,
  },
  every small/.style={/tikzfeynman/small@@/.append style={#1}},
  every small@@/.style={
    /tikz/node distance=1cm,
    /graph drawing/node distance=1.25cm,
    /graph drawing/level distance=1cm,
    /graph drawing/sibling distance=1.5cm,
    /tikzfeynman/every dot@@/.append style={/tikz/minimum size=1mm},
    /tikzfeynman/every crossed dot@@/.append style={/tikz/minimum size=2mm},
    /tikzfeynman/every blob@@/.append style={/tikz/minimum size=0.5cm},
    /tikzfeynman/arrow size=1.2pt,
    /tikzfeynman/insertion/size=2.5pt,
  },
  small/.style={/tikzfeynman/every small@@},
  every medium/.style={/tikzfeynman/medium@@/.append style={#1}},
  every medium@@/.style={
    /tikz/node distance=1.5cm,
    /graph drawing/node distance=1.9cm,
    /graph drawing/level distance=1.5cm,
    /graph drawing/sibling distance=2.25cm,
  },
  medium/.style={/tikzfeynman/every medium@@},
  every large/.style={/tikzfeynman/large@@/.append style={#1}},
  every large@@/.style={
    /tikz/node distance=2cm,
    /graph drawing/node distance=2.5cm,
    /graph drawing/level distance=2cm,
    /graph drawing/sibling distance=3cm,
    /tikz/graphs/edges={thick},
    /tikzfeynman/every dot@@/.append style={/tikz/minimum size=2mm},
    /tikzfeynman/every crossed dot@@/.append style={/tikz/minimum size=4mm},
    /tikzfeynman/every blob@@/.append style={/tikz/minimum size=1cm},
    /tikzfeynman/arrow size=1.6pt,
    /tikzfeynman/insertion/size=4pt,
  },
  large/.style={/tikzfeynman/every large@@},
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Vertices
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every vertex@@/.style={
    /tikz/shape=coordinate,
  },
  every vertex/.style={/tikzfeynman/every vertex@@/.append style={#1}},
  vertex/.style={
    /tikzfeynman/every vertex@@,
  },
  every dot@@/.style={
    /tikz/shape=circle,
    /tikz/graphs/as={},
    /tikz/draw,
    /tikz/fill,
    /tikz/inner sep=0pt,
    /tikz/outer sep=0pt,
    /tikz/minimum size=1.5mm,
  },
  every dot/.style={/tikzfeynman/every dot@@/.append style={#1}},
  dot/.style={
    /tikzfeynman/every dot@@,
  },
  every square dot@@/.style={
    /tikz/shape=rectangle,
  },
  every square dot/.style={/tikzfeynman/every square dot@@/.append style={#1}},
  square dot/.style={
    /tikzfeynman/every dot@@,
    /tikzfeynman/every square dot@@,
  },
  every empty dot@@/.style={
    /tikz/fill=none,
  },
  every empty dot/.style={/tikzfeynman/every empty dot@@/.append style={#1}},
  empty dot/.style={
    /tikzfeynman/every dot@@,
    /tikzfeynman/every empty dot@@,
  },
  every crossed dot@@/.style={
    /tikz/fill=none,
    /tikz/shape=crossed circle,
    /tikz/minimum size=3mm,
  },
  every crossed dot/.style={/tikzfeynman/every crossed dot@@/.append style={#1}},
  crossed dot/.style={
    /tikzfeynman/every dot@@,
    /tikzfeynman/every crossed dot@@,
  },
  every blob@@/.style={
    /tikz/shape=circle,
    /tikz/graphs/as={},
    /tikz/draw,
    /tikz/fill=none,
    /tikz/outer sep=0.5\pgflinewidth,
    /tikz/inner sep=0pt,
    /tikz/minimum size=0.75cm,
    /tikz/pattern=north west lines,
  },
  every blob/.style={/tikzfeynman/every blob@@/.append style={#1}},
  blob/.style={
    /tikzfeynman/every blob@@,
  },
  every particle@@/.style={
    /tikz/shape=rectangle,
    /tikz/draw=none,
    /tikz/fill=none,
    /tikz/inner sep=0.3333em,
    /tikz/outer sep=0.5\pgflinewidth,
  },
  every particle/.style={/tikzfeynman/every particle@@/.append style={#1}},
  particle/.style args={#1}{
    /tikzfeynman/every particle@@,
    /tikz/graphs/as={#1},
  },
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Edge styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Arrow Style
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  arrow size/.store in=\tikzfeynman@arrow@size,
  arrow size=1.5pt,
  with arrow/.style={
    /tikz/decoration={
      markings,
      mark=at position #1 with {
        \node[
          transform shape,
          xshift=-0.5mm,
          fill,
          inner sep=\tikzfeynman@arrow@size,
          draw=none,
          isosceles triangle
        ] { };
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  with reversed arrow/.style={
    /tikz/decoration={
      markings,
      mark=at position #1 with {
        \node[
          transform shape,
          xshift=-0.5mm,
          rotate=180,
          fill,
          inner sep=\tikzfeynman@arrow@size,
          draw=none,
          isosceles triangle
        ] { };
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  %% Base Edge Styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every edge@@/.style={},
  every edge/.style={/tikzfeynman/every edge@@/.append style={#1}},
  %% Specific Styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every plain@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw
    },
  },
  every plain/.style={/tikzfeynman/every plain@@/.append style={#1}},
  plain/.style={
    /tikzfeynman/every plain@@,
  },
  every boson@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/decoration={
        complete sines,
        amplitude=1mm,
        segment length=2mm,
      },
      /tikz/decorate=true,
    },
  },
  every boson/.style={/tikzfeynman/every boson@@/.append style={#1}},
  boson/.style={
    /tikzfeynman/every boson@@,
  },
  every charged boson@@/.style={
    /tikzfeynman/with arrow=0.5,
  },
  every charged boson/.style={/tikzfeynman/every charged boson@@/.append style={#1}},
  charged boson/.style={
    /tikzfeynman/boson,
    /tikzfeynman/every charged boson@@,
  },
  every anti charged boson@@/.style={
    /tikzfeynman/with reversed arrow=0.5,
  },
  every anti charged boson/.style={/tikzfeynman/every anti charged boson@@/.append style={#1}},
  anti charged boson/.style={
    /tikzfeynman/boson,
    /tikzfeynman/every anti charged boson@@,
  },
  every photon@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/decoration={
        complete sines,
        amplitude=1mm,
        segment length=2mm,
      },
      /tikz/decorate=true,
    },
  },
  every photon/.style={/tikzfeynman/every photon@@/.append style={#1}},
  photon/.style={
    /tikzfeynman/every photon@@,
  },
  every scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/dashed,
    },
  },
  every scalar/.style={/tikzfeynman/every scalar@@/.append style={#1}},
  scalar/.style={
    /tikzfeynman/every scalar@@,
  },
  every charged scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikzfeynman/with arrow=0.5,
    },
  },
  every charged scalar/.style={/tikzfeynman/every charged scalar@@/.append style={#1}},
  charged scalar/.style={
    /tikzfeynman/scalar,
    /tikzfeynman/every charged scalar@@,
  },
  every anti charged scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikzfeynman/with reversed arrow=0.5,
    },
  },
  every anti charged scalar/.style={/tikzfeynman/every anti charged scalar@@/.append style={#1}},
  anti charged scalar/.style={
    /tikzfeynman/scalar,
    /tikzfeynman/every anti charged scalar@@,
  },
  every ghost@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/dotted,
      /tikz/thick,
    },
  },
  every ghost/.style={/tikzfeynman/every ghost@@/.append style={#1}},
  ghost/.style={
    /tikzfeynman/every ghost@@,
  },
  every fermion@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynman/with arrow=0.5,
    },
  },
  every fermion/.style={/tikzfeynman/every fermion@@/.append style={#1}},
  fermion/.style={
    /tikzfeynman/every fermion@@,
  },
  every anti fermion@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynman/with reversed arrow=0.5,
    },
  },
  every anti fermion/.style={/tikzfeynman/every anti fermion@@/.append style={#1}},
  anti fermion/.style={
    /tikzfeynman/every anti fermion@@,
  },
  every majorana@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynman/with arrow=0.33,
      /tikzfeynman/with reversed arrow=0.73,
    },
  },
  every majorana/.style={/tikzfeynman/every majorana@@/.append style={#1}},
  majorana/.style={
    /tikzfeynman/every majorana@@,
  },
  every anti majorana@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynman/with reversed arrow=0.33,
      /tikzfeynman/with arrow=0.73,
    },
  },
  every anti majorana/.style={/tikzfeynman/every anti majorana@@/.append style={#1}},
  anti majorana/.style={
    /tikzfeynman/every anti majorana@@,
  },
  every gluon@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/decoration={
        coil,
        aspect=0.75,
        mirror,
        segment length=1.5mm
      },
      /tikz/decorate=true,
    },
  },
  every gluon/.style={/tikzfeynman/every gluon@@/.append style={#1}},
  gluon/.style={
    /tikzfeynman/every gluon@@,
  },
  %% Insertions
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  insertion/.search also={/tikzfeynman,/tikz},
  %% Parameters
  insertion/size/.store in=\tikzfeynman@insertion@size,
  insertion/size=3pt,
  insertion/style/.store in=\tikzfeynman@insertion@style,
  insertion/style={},
  %% Styles
  insertion@@/.style args={[#1]#2}{
    /tikz/decoration={
      markings,
      mark=at position #2 with {
        \tikzfeynmanset{insertion/.cd,#1}
        \draw [\tikzfeynman@insertion@style] (-\tikzfeynman@insertion@size, -\tikzfeynman@insertion@size) -- (\tikzfeynman@insertion@size, \tikzfeynman@insertion@size);
        \draw [\tikzfeynman@insertion@style] (-\tikzfeynman@insertion@size, \tikzfeynman@insertion@size) -- (\tikzfeynman@insertion@size, -\tikzfeynman@insertion@size);
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  insertion@@/.default={[]0.5},
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Momentum arrows
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  momentum/.search also={/tikzfeynman,/tikz},
  %% Parameters
  momentum/label distance/.store in=\tikzfeynman@momentum@label@distance,
  momentum/label distance=0pt,
  momentum/arrow distance/.store in=\tikzfeynman@momentum@arrow@distance,
  momentum/arrow distance=3mm,
  momentum/arrow shorten/.store in=\tikzfeynman@momentum@arrow@shorten,
  momentum/arrow shorten=0.15,
  momentum/label style/.store in=\tikzfeynman@momentum@label@style,
  momentum/label style={},
  momentum/arrow style/.store in=\tikzfeynman@momentum@arrow@style,
  momentum/arrow style={},
  %% Styles
  momentum@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst)
                .. controls (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
                .. (\tikzinputsegmentlast)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynman@momentum@arrow@shorten + (1-2 * \tikzfeynman@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@26)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  momentum'@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst)
                .. controls (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
                .. (\tikzinputsegmentlast)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynman@momentum@arrow@shorten + (1-2 * \tikzfeynman@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@26)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  reversed momentum@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast)
                .. controls (\tikzinputsegmentsupportb) and (\tikzinputsegmentsupporta)
                .. (\tikzinputsegmentfirst)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynman@momentum@arrow@shorten + (1-2 * \tikzfeynman@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@26)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  reversed momentum'@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5,
                      auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast)
                .. controls (\tikzinputsegmentsupportb) and (\tikzinputsegmentsupporta)
                .. (\tikzinputsegmentfirst)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynman@momentum@arrow@shorten + (1-2 * \tikzfeynman@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@26)$)
                node [pos=0.5,
                      auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Modifiers
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  half left/.style={
    /tikz/bend left=90,
    /tikz/looseness=1.5,
  },
  half right/.style={
    /tikz/bend right=90,
    /tikz/looseness=1.5,
  },
  quarter left/.style={
    /tikz/bend left=45,
  },
  quarter right/.style={
    /tikz/bend right=45,
  },
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Graceful Failure of LuaTeX keys
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@luatex@required@path{
  \PackageWarning{tikz-feynman}{The key you tried to use '\pgfkeyscurrentpath/\pgfkeyscurrentname' requires LuaTeX.  It will be ignored.}
}
\def\tikzfeynman@luatex@required@key{
  \PackageWarning{tikz-feynman}{The key you tried to use '\pgfkeyscurrentpath' requires LuaTeX.  It will be ignored.}
}

\ifluatex\else
  \pgfkeys{
    /graph drawing/.unknown/.code=\tikzfeynman@luatex@required@path,
    /tikz/graphs/.unknown/.code=\tikzfeynman@luatex@required@path,
    /tikz/horizontal/.code=\tikzfeynman@luatex@required@key,
    /tikz/horizontal'/.code=\tikzfeynman@luatex@required@key,
    /tikz/vertical/.code=\tikzfeynman@luatex@required@key,
    /tikz/vertical'/.code=\tikzfeynman@luatex@required@key,
    /tikz/tree layout/.code=\tikzfeynman@luatex@required@key,
    /tikz/spring layout/.code=\tikzfeynman@luatex@required@key,
    /tikz/layered layout/.code=\tikzfeynman@luatex@required@key,
    /tikz/spring electrical layout/.code=\tikzfeynman@luatex@required@key,
    /tikz/electric charge/.code=\tikzfeynman@luatex@required@key,
  }
  % \tikzfeynmanset{
  %   horizontal/.code={The key 'horizontal' requires LuaTeX.  It will be ignored.},
  % }
\fi

\endinput

==> Sudakov Shoulders/tikzlibrarypie.code.tex <==
% SPDX-License-Identifier: GPL-2.0-only OR LPPL-1.3c
\RequirePackage{scalefnt}

%
% Utilities
%

\def\pgfpie@ifx#1#2{%
  \ifx#1#2%
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

\def\pgfpie@ifdim#1#2#3{%
  \ifdim\dimexpr#1\relax#2\dimexpr#3\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

\def\pgfpie@ifnum#1#2#3{%
  \ifnum\numexpr#1\relax#2\numexpr#3\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

\def\pgfpie@ifodd#1{%
  \ifodd\numexpr#1\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

\def\pgfpie@newif#1{%
  \csname newif\expandafter\endcsname\csname ifpgfpie@#1\endcsname
  \expandafter\def\csname pgfpie@if#1\expandafter\endcsname\expandafter{%
    \csname ifpgfpie@#1\endcsname
      \expandafter\pgfutil@firstoftwo
    \else
      \expandafter\pgfutil@secondoftwo
    \fi}%
}

%
% Constants for text comparison
%

\def\pgfpie@text@inside{inside}
\def\pgfpie@text@legend{legend}
\def\pgfpie@sum@c{100}
\def\pgfpie@sum@auto{auto}

% args:
% #1: begin angle
% #2: end angle
% #3: number
% #4: label
% #5: explode
% #6: fill color
% #7: radius
% #8: center
\def\pgfpie@slice#1#2#3#4#5#6#7#8{%
  \pgfmathparse{0.5*(#1)+0.5*(#2)}
  \let\pgfpie@midangle\pgfmathresult

  \path (#8) -- ++({\pgfpie@midangle}:{#5}) coordinate (pgfpie@O);

  \pgfmathparse{(#7)+(#5)}
  \let\pgfpie@radius\pgfmathresult
  
  % slice
  \draw[line join=round,fill={#6},\pgfpie@style] (pgfpie@O) -- ++({#1}:{#7}) arc ({#1}:{#2}:{#7}) -- cycle;

  \pgfpie@ifchangedirection{%
    \pgfmathparse{min(((#1)-(#2)-10)/110*(-0.3),0)}
  }{%
    \pgfmathparse{min(((#2)-(#1)-10)/110*(-0.3),0)}
  }%
  
  \pgfmathparse{(max(\pgfmathresult,-0.5) + 0.8)*(#7)}
  \let\pgfpie@innerpos\pgfmathresult

  \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{%
    % label and number together
    \path (pgfpie@O) -- ++({\pgfpie@midangle}:{\pgfpie@innerpos}) node[align=center]
    {\pgfpie@scalefont{#3}\pgfpie@labeltext{#4}\\\pgfpie@numbertext{#3}};
  }{%
    % label
    \pgfpie@ifhidelabel{}{%
      \pgfpie@iflegend{}{%
        \path (pgfpie@O) -- ++ ({\pgfpie@midangle}:{\pgfpie@radius})
        node[inner sep=0, \pgfpie@text={\pgfpie@midangle:#4}]{};
      }%
    }%

    % number
    \path (pgfpie@O) -- ++({\pgfpie@midangle}:{\pgfpie@innerpos}) node
    {\pgfpie@scalefont{#3}\pgfpie@numbertext{#3}};
  }%
}

\def\pgfpie@findColor#1{%
  \pgfmathparse{int(mod(#1,\the\pgfpie@colorLength))}%
  \let\pgfpie@ci\pgfmathresult
  \foreach \pgfpie@c [count=\pgfpie@j from 0] in \pgfpie@color {%
    \pgfpie@ifnum{\pgfpie@j}{=}{\pgfpie@ci}{%
      \xdef\pgfpie@thecolor{\pgfpie@c}%
      \breakforeach
    }{}%
  }
}

\def\pgfpie@findExplode#1{%
  \pgfmathparse{int(mod(#1,\the\pgfpie@explodeLength))}%
  \let\pgfpie@ei\pgfmathresult
  \foreach \pgfpie@e [count=\pgfpie@j from 0] in \pgfpie@explode {%
    \pgfpie@ifnum{\pgfpie@j}{=}{\pgfpie@ei}{%
      \xdef\pgfpie@theexplode{\pgfpie@e}%
      \breakforeach
    }{}%
  }%
}

% #1: bottom left point
% #2: size
% #3: number
% #4: color
% #5: text
\def\pgfpie@square#1#2#3#4#5{%
  \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{%
    \draw[fill={#4},\pgfpie@style] (#1) rectangle node[align=center]
    {\pgfpie@scalefont{#3}\pgfpie@labeltext{#5}\\\pgfpie@numbertext{#3}} ++(#2);
  }{%
    \draw[fill={#4},\pgfpie@style] (#1) rectangle node
    {\pgfpie@scalefont{#3}\pgfpie@numbertext{#3}} ++(#2);
  }%
}

% #1: pos
% #2: radius
% #3: number
% #4: color
% $5: style
% $6: label
\def\pgfpie@cloud#1#2#3#4#5#6{%
  \draw[fill=#4, #5] (#1) circle[radius=#2];
  \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{%
    \node[align=center] at (#1) {\pgfpie@scalefont{#3}\pgfpie@labeltext{#6}\\\pgfpie@numbertext{#3}};
  }{%
    \node at (#1) {\pgfpie@scalefont{#3}\pgfpie@numbertext{#3}};
  }%
}

\newdimen\pgfpie@angleEnd
\newcount\pgfpie@explodeLength
\newcount\pgfpie@colorLength
\newcount\pgfpie@sliceLength

\pgfqkeys{/pgfpie}{%
  .search also={/tikz,/pgf},
  explode/.store in=\pgfpie@explode,
  color/.store in=\pgfpie@color,
  radius/.store in=\pgfpie@radius,
  pos/.store in=\pgfpie@pos,
  style/.store in=\pgfpie@style,
  before number/.store in=\pgfpie@beforenumber,
  after number/.code={%
    \def\pgfpie@afternumber{#1}%
    \def\pgfpie@late@afternumber{}%
  },
  text/.store in=\pgfpie@text,
  sum/.code={%
    \def\pgfpie@sum{#1}%
    \pgfpie@ifx\pgfpie@sum\pgfpie@sum@c{%
      \def\pgfpie@late@afternumber{\def\pgfpie@afternumber{\%}}%
    }{%
      \def\pgfpie@late@afternumber{}%
    }%
  },
  rotate/.store in=\pgfpie@rotate,
}

\pgfpie@newif{polar}
\pgfqkeys{/pgfpie}{polar/.is if=pgfpie@polar}

\pgfpie@newif{legend}

\pgfpie@newif{changedirection}
\pgfqkeys{/pgfpie}{change direction/.is if=pgfpie@changedirection}

\pgfpie@newif{square}
\pgfqkeys{/pgfpie}{square/.is if=pgfpie@square}

\pgfpie@newif{cloud}
\pgfqkeys{/pgfpie}{cloud/.is if=pgfpie@cloud}

\pgfpie@newif{scalefont}
\pgfqkeys{/pgfpie}{scale font/.is if=pgfpie@scalefont}
\def\pgfpie@scalefont#1{%
  \pgfpie@ifscalefont{%
    \pgfmathparse{(#1) / (\pgfpie@sum) * 3 + 0.9}%
    \scalefont{\pgfmathresult}%
  }{}%
}

\pgfpie@newif{hidenumber}
\pgfqkeys{/pgfpie}{hide number/.is if=pgfpie@hidenumber}
\def\pgfpie@numbertext#1{%
  \pgfpie@ifhidenumber{}{%
    \pgfpie@beforenumber#1\pgfpie@afternumber
  }%
}

\pgfpie@newif{hidelabel}
\pgfqkeys{/pgfpie}{hide label/.is if=pgfpie@hidelabel}
\def\pgfpie@labeltext#1{\pgfpie@ifhidelabel{}{#1}}

\tikzaddtikzonlycommandshortcutlet{\pie}{\pgfpie@pie}%

\def\pgfpie@pie{%
  \pgfutil@ifnextchar[{\pgfpie@@pie}{\pgfpie@@pie[]}%
}

\def\pgfpie@@pie[#1]#2{%
  \scope[%
    % to be compatible with "babel" lib
    handle active characters in nodes=false,
    % load default parameters
    /pgfpie/.cd,
    explode=0,
    color={blue!60, cyan!60, yellow!60, orange!60, red!60,
      blue!60!cyan!60, cyan!60!yellow!60, red!60!cyan!60,
      red!60!blue!60, orange!60!cyan!60},
    radius=3,
    pos={0,0},
    style={thick},
    before number=,
    after number=,
    text=label,
    sum=100,
    rotate=0,
    change direction=false,
    polar=false,
    square=false,
    cloud=false,
    scale font=false,
    hide number=false,
    hide label=false,
    every pie/.try,%
    % load user's parameters
    #1]

  % add percentage automatically
  \pgfpie@late@afternumber

  % legend or not
  \pgfpie@ifx\pgfpie@text\pgfpie@text@legend{%
    \pgfpie@legendtrue
  }{%
    \pgfpie@legendfalse
  }%

  % handle sum
  \pgfpie@ifx\pgfpie@sum\pgfpie@sum@auto{%
    % sum all input
    \xdef\pgfpie@sum{0}%
    \foreach \pgfpie@p/\pgfpie@t in {#2} {%
      \pgfmathparse{(\pgfpie@sum) + (\pgfpie@p)}%
      \xdef\pgfpie@sum{\pgfmathresult}%
    }%
  }{}%

  % init counters
  \global\pgfpie@explodeLength=0
  \foreach \pgfpie@e in \pgfpie@explode {%
    \global\advance\pgfpie@explodeLength by 1
  }%

  \global\pgfpie@colorLength=0
  \foreach \pgfpie@c in \pgfpie@color {%
    \global\advance\pgfpie@colorLength by 1
  }%
  
  \pgfmathsetlength{\pgfpie@angleEnd}{0}%

  \global\pgfpie@sliceLength=0
  \foreach \pgfpie@p/\pgfpie@e in {#2} {%
    \global\advance\pgfpie@sliceLength by 1
  }%

  \pgfpie@ifsquare{%
    \pgfpie@pie@square{#2}%
    }{\pgfpie@ifcloud{\pgfpie@pie@cloud{#2}%
      }{\pgfpie@pie@circle{#2}}}

  % legend
  \pgfpie@ifhidelabel{}{%
    \pgfpie@iflegend{%
      \pgfpie@legend{#2}%
  }{}}%
  \endscope
}

\def\pgfpie@pie@square#1{%
  \pgfmathparse{(\pgfpie@radius)*2}
  \xdef\pgfpie@verticalLength{\pgfmathresult}
  \xdef\pgfpie@horizontalLength{\pgfmathresult}
  \path (\pgfpie@pos) -- ++({-\pgfpie@radius},{-\pgfpie@radius}) coordinate (pgfpie@start);
  \pgfmathparse{(\pgfpie@verticalLength) * (\pgfpie@horizontalLength) / (\pgfpie@sum)}
  \let\pgfpie@squareUnit\pgfmathresult

  % drawing loop
  \foreach \pgfpie@p/\pgfpie@t [count=\pgfpie@i from 0] in {#1}
  {
    \pgfpie@findColor{\pgfpie@i}

    \pgfpie@ifdim{\pgfpie@verticalLength cm}{>}{\pgfpie@horizontalLength cm}{%
      \pgfmathparse{(\pgfpie@p) * (\pgfpie@squareUnit) / (\pgfpie@horizontalLength)}
      \let\pgfpie@height\pgfmathresult
      
      \pgfpie@square{pgfpie@start}{\pgfpie@horizontalLength,\pgfpie@height}
      {\pgfpie@p}
      {\pgfpie@thecolor}
      {\pgfpie@t}
      %label
      \pgfpie@iflegend{}{%
        \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{}{%
          \pgfpie@ifhidelabel{}{%
            \path (pgfpie@start) -- ++({\pgfpie@horizontalLength},{\pgfpie@height*0.5})
            node[inner sep=0, \pgfpie@text={0:{\pgfpie@t}}]{};
          }%
        }%
      }%

      \pgfmathparse{\pgfpie@verticalLength - \pgfpie@height}
      \xdef\pgfpie@verticalLength{\pgfmathresult}
      \path (pgfpie@start) -- ++(0, \pgfpie@height) coordinate (pgfpie@start);
    }{%
      \pgfmathparse{(\pgfpie@p) * (\pgfpie@squareUnit) / (\pgfpie@verticalLength)}%
      \let\pgfpie@width\pgfmathresult

      \pgfpie@square{pgfpie@start}{\pgfpie@width,\pgfpie@verticalLength}
      {\pgfpie@p}
      {\pgfpie@thecolor}
      {\pgfpie@t}
      %label
      \pgfpie@iflegend{}{%
        \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{}{%
          \pgfpie@ifhidelabel{}{%
            \path (pgfpie@start) -- ++({\pgfpie@width*0.5},{\pgfpie@verticalLength})
            node[inner sep=0, \pgfpie@text={90:{\pgfpie@t}}]{};
          }%
        }%
      }%

      \pgfmathparse{(\pgfpie@horizontalLength) - (\pgfpie@width)}%
      \xdef\pgfpie@horizontalLength{\pgfmathresult}%
      \path (pgfpie@start) -- ++({\pgfpie@width},0) coordinate (pgfpie@start);
    }%
  }%
}

\def\pgfpie@pie@cloud#1{%
  % drawing loop
  \foreach \pgfpie@p/\pgfpie@t [count=\pgfpie@i from 0] in {#1}
  {
    % find explode
    \pgfpie@findExplode{\pgfpie@i}
    \def\pgfpie@cloudGap{(\pgfpie@theexplode) + 0.1}
    \pgfmathparse{sqrt((\pgfpie@p) / (\pgfpie@sum)) * (\pgfpie@radius)}
    \let\pgfpie@cloudR\pgfmathresult
    \pgfpie@ifnum{\pgfpie@i}{=}{0}{%
      % first cloud
      \coordinate (pgfpie@O) at (\pgfpie@pos);
      \xdef\pgfpie@cloudRone{\pgfpie@cloudR}
      \xdef\pgfpie@cloudExtendDir{180+(\pgfpie@rotate)}
    }{\pgfpie@ifnum{\pgfpie@i}{=}{1}{%
      % second cloud
      \xdef\pgfpie@cloudRtwo{\pgfpie@cloudR}
      \xdef\pgfpie@cloudExtendDir{45+(\pgfpie@rotate)}
      \path (pgfpie@O) -- ++({\pgfpie@cloudExtendDir}:{(\pgfpie@cloudRone)+(\pgfpie@cloudGap)+(\pgfpie@cloudRtwo)}) coordinate (pgfpie@O);
    }{%
      % next cloud
      \pgfmathparse{(\pgfpie@cloudRone)+(\pgfpie@cloudGap)+(\pgfpie@cloudRtwo)}
      \let\pgfpie@la\pgfmathresult
      \pgfmathparse{(\pgfpie@cloudRone)+(\pgfpie@cloudGap)+(\pgfpie@cloudR)}
      \let\pgfpie@lb\pgfmathresult
      \pgfmathparse{(\pgfpie@cloudRtwo)+(\pgfpie@cloudGap)+(\pgfpie@cloudR)}
      \let\pgfpie@lc\pgfmathresult
      \pgfmathparse{(\pgfpie@la)^2+(\pgfpie@lc)^2-(\pgfpie@lb)^2}
      \let\pgfpie@tmp\pgfmathresult
      \pgfmathparse{180 - acos((\pgfpie@tmp) / 2 / (\pgfpie@la) / (\pgfpie@lc))}
      \let\pgfpie@cloudRot\pgfmathresult
      \pgfpie@ifodd{\pgfpie@i}{%
        \pgfmathparse{-(\pgfpie@cloudRot)}
        \let\pgfpie@cloudRot\pgfmathresult
      }{}%
      \pgfmathparse{(\pgfpie@cloudExtendDir) - (\pgfpie@cloudRot)}
      \xdef\pgfpie@cloudExtendDir{\pgfmathresult}
      \path (pgfpie@O) -- ++({\pgfpie@cloudExtendDir}:{\pgfpie@lc}) coordinate (pgfpie@O);
      \xdef\pgfpie@cloudRone{\pgfpie@cloudRtwo}
      \xdef\pgfpie@cloudRtwo{\pgfpie@cloudR}
    }}%

    % find color
    \pgfpie@findColor{\pgfpie@i}

    \pgfpie@cloud{pgfpie@O}{\pgfpie@cloudR}{\pgfpie@p}
    {\pgfpie@thecolor}{\pgfpie@style}{\pgfpie@t}

    % label
    \pgfpie@iflegend{}{%
      \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{}{%
        \pgfpie@ifhidelabel{}{%
          \path (pgfpie@O) -- ++({\pgfpie@cloudExtendDir}:{\pgfpie@cloudR})
          node[inner sep=0, \pgfpie@text={\pgfpie@cloudExtendDir:{\pgfpie@t}}] {};
        }%
      }%
    }%
  }%
}

\def\pgfpie@pie@circle#1{%
  \pgfpie@ifpolar{%
    \xdef\pgfpie@maxValue{0}
    \foreach \pgfpie@p/\pgfpie@e in {#1} {
      \pgfmathparse{\pgfpie@p}%
      \pgfpie@ifdim{\pgfpie@maxValue pt}{<}{\pgfmathresult pt}{%
        \xdef\pgfpie@maxValue{\pgfpie@p}
      }{}%
    }
    \pgfmathparse{(\pgfpie@sum) / \the\pgfpie@sliceLength}
    \xdef\pgfpie@polarangle{\pgfmathresult}
    \pgfmathparse{(\pgfpie@radius) / sqrt(\pgfpie@maxValue)}
    \xdef\pgfpie@polarRadiusUnit{\pgfmathresult}
  }{%
    \xdef\pgfpie@theradius{\pgfpie@radius}%
  }

  \pgfpie@ifchangedirection{%
    \pgfmathsetlength{\pgfpie@angleEnd}{\pgfpie@sum}
  }{}%
  \xdef\pgfpie@angleBegin{\the\pgfpie@angleEnd}
  % drawing loop
  \foreach \pgfpie@p/\pgfpie@t [count=\pgfpie@i from 0] in {#1}
  {
    \pgfmathsetlength{\pgfpie@angleEnd}{\pgfpie@angleBegin}
    \pgfpie@ifpolar{%
      % Polar area diagram
      \pgfmathaddtolength{\pgfpie@angleEnd}{\pgfpie@polarangle}
      \pgfmathparse{sqrt(\pgfpie@p) * (\pgfpie@polarRadiusUnit)}
      \xdef\pgfpie@theradius{\pgfmathresult}
    }{%
      % normal pie
      \pgfpie@ifchangedirection{%
        \pgfmathaddtolength{\pgfpie@angleEnd}{-(\pgfpie@p)}
      }{%
        \pgfmathaddtolength{\pgfpie@angleEnd}{\pgfpie@p}
      }%
    }%

    % find explode
    \pgfpie@findExplode{\pgfpie@i}

    % find color
    \pgfpie@findColor{\pgfpie@i}
    \pgfpie@slice{(\pgfpie@angleBegin)/(\pgfpie@sum)*360+(\pgfpie@rotate)}
    {\the\pgfpie@angleEnd/(\pgfpie@sum)*360+(\pgfpie@rotate)}
    {\pgfpie@p}
    {\pgfpie@t}
    {\pgfpie@theexplode}
    {\pgfpie@thecolor}
    {\pgfpie@theradius}
    {\pgfpie@pos}
    \xdef\pgfpie@angleBegin{\the\pgfpie@angleEnd}
  }
}

\def\pgfpie@legend#1{%
  \coordinate[xshift=0.8cm,
  yshift={(\the\pgfpie@sliceLength*0.5+1)*0.5cm}] (pgfpie@legendpos) at
  (current bounding box.east);

  \scope[node distance=0.5cm]
    \foreach \pgfpie@p/\pgfpie@t [count=\pgfpie@i from 0] in {#1}
    {
      \pgfpie@findColor{\pgfpie@i}
      \node[draw, fill={\pgfpie@thecolor}, \pgfpie@style, below of={pgfpie@legendpos}, label={0:{\pgfpie@t}}] (pgfpie@legendpos) {};
    }
  \endscope
}


==> tikzfeynman.keys.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% TikZ-Feynman
% Feynman Diagrams with TikZ
% Copyright (C) 2015  Joshua Ellis
%
%
% This work may be distributed and/or modified under the terms of the GNU General
% Public License as published by the Free Software Foundation, either version 3 
% of the License, or (at your option) any later version.
%
% This program is distributed in the hope that it will be useful, but WITHOUT
% ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or FITNESS
% FOR A PARTICULAR PURPOSE.  See the LaTeX Project Public License for more
% details.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Shapes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Crossed Circle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclareshape{crossed circle}
{
  \inheritsavedanchors[from=circle]
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}

  \inheritbackgroundpath[from=circle]

  \foregroundpath{
    % Compute south west
    \centerpoint
    \pgf@xc=\radius
    \advance\pgf@x by-0.707107\pgf@xc
    \advance\pgf@y by-0.707107\pgf@xc
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y  % Store coordinates
    % Compute north east point
    \centerpoint
    \pgf@xc=\radius
    \advance\pgf@x by0.707107\pgf@xc
    \advance\pgf@y by0.707107\pgf@xc
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y  % Store coordinates
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
    \pgfsetarrowsstart{}
    \pgfsetarrowsend{}
 }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Decorations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Complete Sines
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Complete sines replaces the path with a whole number of sine waves.
%% Thanks to http://tex.stackexchange.com/a/134516/26980
\pgfdeclaredecoration{complete sines}{initial}
{
  %% Begin by computing the overall path length and find how many sine waves we
  %% can fit in.  Nothing happens beyond the computation.
  \state{initial}[
    width=+0pt,
    next state=move,
    persistent precomputation={
      \def\tikzfeynman@cs@angle@step{30}
      \def\tikzfeynman@cs@current@angle{0}
      \pgfmathsetlengthmacro{\tikzfeynman@cs@points@per@step}{
        \pgfdecoratedinputsegmentlength
        / int(\pgfdecoratedinputsegmentlength
        / \pgfdecorationsegmentlength)
        / 360
        * \tikzfeynman@cs@angle@step}
    },
  ]{}
  %% Move to the origin to the path
  \state{move}[
    width=+\tikzfeynman@cs@points@per@step,
    next state=draw
  ]{
    \pgfpathmoveto{\pgfpointorigin}
  }
  %% Draw the sine wave itself.  This computes the value every 20 degrees and draws straight edges.
  \state{draw}[
    width=+\tikzfeynman@cs@points@per@step,
    switch if less than=1.25*\tikzfeynman@cs@points@per@step to final, % <- bit of a hack
    persistent postcomputation={
      \pgfmathparse{mod(\tikzfeynman@cs@current@angle+\tikzfeynman@cs@angle@step, 360)}
      \let\tikzfeynman@cs@current@angle=\pgfmathresult%
    },
  ]{
    \pgfmathparse{sin(\tikzfeynman@cs@current@angle) * \pgfmetadecorationsegmentamplitude / 2}
    \tikz@decoratepathfalse
    \pgfpathlineto{\pgfqpoint{0pt}{\pgfmathresult pt}}%
  }

  \state{final}{
    \ifdim\pgfdecoratedremainingdistance>0pt\relax
      \pgfpathlineto{\pgfpointdecoratedpathlast}
    \fi
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Keys
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzfeynmanset{
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Hooks
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  execute at begin feynman/.code={},
  execute at end feynman/.code={},
  every feynman/.style={/tikzfeynman/every feynman@@/.append style={#1}},
  every feynman@@/.style={
    /tikzfeynman/.cd,
    /tikzfeynman/medium,
  },
  execute at begin feynman@@/.code={}                     %% Internal version
  execute at end feynman@@/.code={},                      %% Internal version
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Diagrams
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every diagram/.style={/tikzfeynman/every diagram@@/.append style={#1}},
  every diagram@@/.style={
    /tikzfeynman/.cd,
    .search also={/tikz/graphs, /tikz},
    nodes={
      /tikzfeynman/.cd,
      /tikzfeynman/.search also={/tikz/graphs, /tikz},
      /tikzfeynman/every vertex@@,
      /tikzfeynman/every vertex},
    edges={
      /tikzfeynman/.cd,
      /tikzfeynman/.search also={/tikz/graphs, /tikz},
      /tikzfeynman/every edge@@,
      /tikzfeynman/every edge},
    /tikzfeynman/medium,
  },
  every inline/.style={/tikzfeynman/inline@@/.append style={#1}},
  every inline@@/.style={
    /tikzfeynman/small,
  },
  inline/.style={
    /tikz/baseline={#1},
    /tikzfeynman/every inline@@,
  },
  every small/.style={/tikzfeynman/small@@/.append style={#1}},
  every small@@/.style={
    /tikz/node distance=1cm,
    /graph drawing/node distance=1.25cm,
    /graph drawing/level distance=1cm,
    /graph drawing/sibling distance=1.5cm,
    /tikzfeynman/every dot@@/.append style={/tikz/minimum size=1mm},
    /tikzfeynman/every crossed dot@@/.append style={/tikz/minimum size=2mm},
    /tikzfeynman/every blob@@/.append style={/tikz/minimum size=0.5cm},
    /tikzfeynman/arrow size=1.2pt,
    /tikzfeynman/insertion/size=2.5pt,
  },
  small/.style={/tikzfeynman/every small@@},
  every medium/.style={/tikzfeynman/medium@@/.append style={#1}},
  every medium@@/.style={
    /tikz/node distance=1.5cm,
    /graph drawing/node distance=1.9cm,
    /graph drawing/level distance=1.5cm,
    /graph drawing/sibling distance=2.25cm,
  },
  medium/.style={/tikzfeynman/every medium@@},
  every large/.style={/tikzfeynman/large@@/.append style={#1}},
  every large@@/.style={
    /tikz/node distance=2cm,
    /graph drawing/node distance=2.5cm,
    /graph drawing/level distance=2cm,
    /graph drawing/sibling distance=3cm,
    /tikz/graphs/edges={thick},
    /tikzfeynman/every dot@@/.append style={/tikz/minimum size=2mm},
    /tikzfeynman/every crossed dot@@/.append style={/tikz/minimum size=4mm},
    /tikzfeynman/every blob@@/.append style={/tikz/minimum size=1cm},
    /tikzfeynman/arrow size=1.6pt,
    /tikzfeynman/insertion/size=4pt,
  },
  large/.style={/tikzfeynman/every large@@},
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Vertices
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every vertex@@/.style={
    /tikz/shape=coordinate,
  },
  every vertex/.style={/tikzfeynman/every vertex@@/.append style={#1}},
  vertex/.style={
    /tikzfeynman/every vertex@@,
  },
  every dot@@/.style={
    /tikz/shape=circle,
    /tikz/graphs/as={},
    /tikz/draw,
    /tikz/fill,
    /tikz/inner sep=0pt,
    /tikz/outer sep=0pt,
    /tikz/minimum size=1.5mm,
  },
  every dot/.style={/tikzfeynman/every dot@@/.append style={#1}},
  dot/.style={
    /tikzfeynman/every dot@@,
  },
  every square dot@@/.style={
    /tikz/shape=rectangle,
  },
  every square dot/.style={/tikzfeynman/every square dot@@/.append style={#1}},
  square dot/.style={
    /tikzfeynman/every dot@@,
    /tikzfeynman/every square dot@@,
  },
  every empty dot@@/.style={
    /tikz/fill=none,
  },
  every empty dot/.style={/tikzfeynman/every empty dot@@/.append style={#1}},
  empty dot/.style={
    /tikzfeynman/every dot@@,
    /tikzfeynman/every empty dot@@,
  },
  every crossed dot@@/.style={
    /tikz/fill=none,
    /tikz/shape=crossed circle,
    /tikz/minimum size=3mm,
  },
  every crossed dot/.style={/tikzfeynman/every crossed dot@@/.append style={#1}},
  crossed dot/.style={
    /tikzfeynman/every dot@@,
    /tikzfeynman/every crossed dot@@,
  },
  every blob@@/.style={
    /tikz/shape=circle,
    /tikz/graphs/as={},
    /tikz/draw,
    /tikz/fill=none,
    /tikz/outer sep=0.5\pgflinewidth,
    /tikz/inner sep=0pt,
    /tikz/minimum size=0.75cm,
    /tikz/pattern=north west lines,
  },
  every blob/.style={/tikzfeynman/every blob@@/.append style={#1}},
  blob/.style={
    /tikzfeynman/every blob@@,
  },
  every particle@@/.style={
    /tikz/shape=rectangle,
    /tikz/draw=none,
    /tikz/fill=none,
    /tikz/inner sep=0.3333em,
    /tikz/outer sep=0.5\pgflinewidth,
  },
  every particle/.style={/tikzfeynman/every particle@@/.append style={#1}},
  particle/.style args={#1}{
    /tikzfeynman/every particle@@,
    /tikz/graphs/as={#1},
  },
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Edge styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Arrow Style
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  arrow size/.store in=\tikzfeynman@arrow@size,
  arrow size=1.5pt,
  with arrow/.style={
    /tikz/decoration={
      markings,
      mark=at position #1 with {
        \node[
          transform shape,
          xshift=-0.5mm,
          fill,
          inner sep=\tikzfeynman@arrow@size,
          draw=none,
          isosceles triangle
        ] { };
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  with reversed arrow/.style={
    /tikz/decoration={
      markings,
      mark=at position #1 with {
        \node[
          transform shape,
          xshift=-0.5mm,
          rotate=180,
          fill,
          inner sep=\tikzfeynman@arrow@size,
          draw=none,
          isosceles triangle
        ] { };
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  %% Base Edge Styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every edge@@/.style={},
  every edge/.style={/tikzfeynman/every edge@@/.append style={#1}},
  %% Specific Styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every plain@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw
    },
  },
  every plain/.style={/tikzfeynman/every plain@@/.append style={#1}},
  plain/.style={
    /tikzfeynman/every plain@@,
  },
  every boson@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/decoration={
        complete sines,
        amplitude=1mm,
        segment length=2mm,
      },
      /tikz/decorate=true,
    },
  },
  every boson/.style={/tikzfeynman/every boson@@/.append style={#1}},
  boson/.style={
    /tikzfeynman/every boson@@,
  },
  every charged boson@@/.style={
    /tikzfeynman/with arrow=0.5,
  },
  every charged boson/.style={/tikzfeynman/every charged boson@@/.append style={#1}},
  charged boson/.style={
    /tikzfeynman/boson,
    /tikzfeynman/every charged boson@@,
  },
  every anti charged boson@@/.style={
    /tikzfeynman/with reversed arrow=0.5,
  },
  every anti charged boson/.style={/tikzfeynman/every anti charged boson@@/.append style={#1}},
  anti charged boson/.style={
    /tikzfeynman/boson,
    /tikzfeynman/every anti charged boson@@,
  },
  every photon@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/decoration={
        complete sines,
        amplitude=1mm,
        segment length=2mm,
      },
      /tikz/decorate=true,
    },
  },
  every photon/.style={/tikzfeynman/every photon@@/.append style={#1}},
  photon/.style={
    /tikzfeynman/every photon@@,
  },
  every scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/dashed,
    },
  },
  every scalar/.style={/tikzfeynman/every scalar@@/.append style={#1}},
  scalar/.style={
    /tikzfeynman/every scalar@@,
  },
  every charged scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikzfeynman/with arrow=0.5,
    },
  },
  every charged scalar/.style={/tikzfeynman/every charged scalar@@/.append style={#1}},
  charged scalar/.style={
    /tikzfeynman/scalar,
    /tikzfeynman/every charged scalar@@,
  },
  every anti charged scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikzfeynman/with reversed arrow=0.5,
    },
  },
  every anti charged scalar/.style={/tikzfeynman/every anti charged scalar@@/.append style={#1}},
  anti charged scalar/.style={
    /tikzfeynman/scalar,
    /tikzfeynman/every anti charged scalar@@,
  },
  every ghost@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/dotted,
      /tikz/thick,
    },
  },
  every ghost/.style={/tikzfeynman/every ghost@@/.append style={#1}},
  ghost/.style={
    /tikzfeynman/every ghost@@,
  },
  every fermion@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynman/with arrow=0.5,
    },
  },
  every fermion/.style={/tikzfeynman/every fermion@@/.append style={#1}},
  fermion/.style={
    /tikzfeynman/every fermion@@,
  },
  every anti fermion@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynman/with reversed arrow=0.5,
    },
  },
  every anti fermion/.style={/tikzfeynman/every anti fermion@@/.append style={#1}},
  anti fermion/.style={
    /tikzfeynman/every anti fermion@@,
  },
  every majorana@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynman/with arrow=0.33,
      /tikzfeynman/with reversed arrow=0.73,
    },
  },
  every majorana/.style={/tikzfeynman/every majorana@@/.append style={#1}},
  majorana/.style={
    /tikzfeynman/every majorana@@,
  },
  every anti majorana@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynman/with reversed arrow=0.33,
      /tikzfeynman/with arrow=0.73,
    },
  },
  every anti majorana/.style={/tikzfeynman/every anti majorana@@/.append style={#1}},
  anti majorana/.style={
    /tikzfeynman/every anti majorana@@,
  },
  every gluon@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/decoration={
        coil,
        aspect=0.75,
        mirror,
        segment length=1.5mm
      },
      /tikz/decorate=true,
    },
  },
  every gluon/.style={/tikzfeynman/every gluon@@/.append style={#1}},
  gluon/.style={
    /tikzfeynman/every gluon@@,
  },
  %% Insertions
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  insertion/.search also={/tikzfeynman,/tikz},
  %% Parameters
  insertion/size/.store in=\tikzfeynman@insertion@size,
  insertion/size=3pt,
  insertion/style/.store in=\tikzfeynman@insertion@style,
  insertion/style={},
  %% Styles
  insertion@@/.style args={[#1]#2}{
    /tikz/decoration={
      markings,
      mark=at position #2 with {
        \tikzfeynmanset{insertion/.cd,#1}
        \draw [\tikzfeynman@insertion@style] (-\tikzfeynman@insertion@size, -\tikzfeynman@insertion@size) -- (\tikzfeynman@insertion@size, \tikzfeynman@insertion@size);
        \draw [\tikzfeynman@insertion@style] (-\tikzfeynman@insertion@size, \tikzfeynman@insertion@size) -- (\tikzfeynman@insertion@size, -\tikzfeynman@insertion@size);
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  insertion@@/.default={[]0.5},
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Momentum arrows
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  momentum/.search also={/tikzfeynman,/tikz},
  %% Parameters
  momentum/label distance/.store in=\tikzfeynman@momentum@label@distance,
  momentum/label distance=0pt,
  momentum/arrow distance/.store in=\tikzfeynman@momentum@arrow@distance,
  momentum/arrow distance=3mm,
  momentum/arrow shorten/.store in=\tikzfeynman@momentum@arrow@shorten,
  momentum/arrow shorten=0.15,
  momentum/label style/.store in=\tikzfeynman@momentum@label@style,
  momentum/label style={},
  momentum/arrow style/.store in=\tikzfeynman@momentum@arrow@style,
  momentum/arrow style={},
  %% Styles
  momentum@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst)
                .. controls (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
                .. (\tikzinputsegmentlast)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynman@momentum@arrow@shorten + (1-2 * \tikzfeynman@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@26)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  momentum'@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst)
                .. controls (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
                .. (\tikzinputsegmentlast)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynman@momentum@arrow@shorten + (1-2 * \tikzfeynman@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@26)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  reversed momentum@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast)
                .. controls (\tikzinputsegmentsupportb) and (\tikzinputsegmentsupporta)
                .. (\tikzinputsegmentfirst)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynman@momentum@arrow@shorten + (1-2 * \tikzfeynman@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@26)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  reversed momentum'@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5,
                      auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast)
                .. controls (\tikzinputsegmentsupportb) and (\tikzinputsegmentsupporta)
                .. (\tikzinputsegmentfirst)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynman@momentum@arrow@shorten + (1-2 * \tikzfeynman@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@26)$)
                node [pos=0.5,
                      auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Modifiers
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  half left/.style={
    /tikz/bend left=90,
    /tikz/looseness=1.5,
  },
  half right/.style={
    /tikz/bend right=90,
    /tikz/looseness=1.5,
  },
  quarter left/.style={
    /tikz/bend left=45,
  },
  quarter right/.style={
    /tikz/bend right=45,
  },
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Graceful Failure of LuaTeX keys
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@luatex@required@path{
  \PackageWarning{tikz-feynman}{The key you tried to use '\pgfkeyscurrentpath/\pgfkeyscurrentname' requires LuaTeX.  It will be ignored.}
}
\def\tikzfeynman@luatex@required@key{
  \PackageWarning{tikz-feynman}{The key you tried to use '\pgfkeyscurrentpath' requires LuaTeX.  It will be ignored.}
}

\ifluatex\else
  \pgfkeys{
    /graph drawing/.unknown/.code=\tikzfeynman@luatex@required@path,
    /tikz/graphs/.unknown/.code=\tikzfeynman@luatex@required@path,
    /tikz/horizontal/.code=\tikzfeynman@luatex@required@key,
    /tikz/horizontal'/.code=\tikzfeynman@luatex@required@key,
    /tikz/vertical/.code=\tikzfeynman@luatex@required@key,
    /tikz/vertical'/.code=\tikzfeynman@luatex@required@key,
    /tikz/tree layout/.code=\tikzfeynman@luatex@required@key,
    /tikz/spring layout/.code=\tikzfeynman@luatex@required@key,
    /tikz/layered layout/.code=\tikzfeynman@luatex@required@key,
    /tikz/spring electrical layout/.code=\tikzfeynman@luatex@required@key,
    /tikz/electric charge/.code=\tikzfeynman@luatex@required@key,
  }
  % \tikzfeynmanset{
  %   horizontal/.code={The key 'horizontal' requires LuaTeX.  It will be ignored.},
  % }
\fi

\endinput

==> tikzlibrarypie.code.tex <==
% SPDX-License-Identifier: GPL-2.0-only OR LPPL-1.3c
\RequirePackage{scalefnt}

%
% Utilities
%

\def\pgfpie@ifx#1#2{%
  \ifx#1#2%
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

\def\pgfpie@ifdim#1#2#3{%
  \ifdim\dimexpr#1\relax#2\dimexpr#3\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

\def\pgfpie@ifnum#1#2#3{%
  \ifnum\numexpr#1\relax#2\numexpr#3\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

\def\pgfpie@ifodd#1{%
  \ifodd\numexpr#1\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

\def\pgfpie@newif#1{%
  \csname newif\expandafter\endcsname\csname ifpgfpie@#1\endcsname
  \expandafter\def\csname pgfpie@if#1\expandafter\endcsname\expandafter{%
    \csname ifpgfpie@#1\endcsname
      \expandafter\pgfutil@firstoftwo
    \else
      \expandafter\pgfutil@secondoftwo
    \fi}%
}

%
% Constants for text comparison
%

\def\pgfpie@text@inside{inside}
\def\pgfpie@text@legend{legend}
\def\pgfpie@sum@c{100}
\def\pgfpie@sum@auto{auto}

% args:
% #1: begin angle
% #2: end angle
% #3: number
% #4: label
% #5: explode
% #6: fill color
% #7: radius
% #8: center
\def\pgfpie@slice#1#2#3#4#5#6#7#8{%
  \pgfmathparse{0.5*(#1)+0.5*(#2)}
  \let\pgfpie@midangle\pgfmathresult

  \path (#8) -- ++({\pgfpie@midangle}:{#5}) coordinate (pgfpie@O);

  \pgfmathparse{(#7)+(#5)}
  \let\pgfpie@radius\pgfmathresult
  
  % slice
  \draw[line join=round,fill={#6},\pgfpie@style] (pgfpie@O) -- ++({#1}:{#7}) arc ({#1}:{#2}:{#7}) -- cycle;

  \pgfpie@ifchangedirection{%
    \pgfmathparse{min(((#1)-(#2)-10)/110*(-0.3),0)}
  }{%
    \pgfmathparse{min(((#2)-(#1)-10)/110*(-0.3),0)}
  }%
  
  \pgfmathparse{(max(\pgfmathresult,-0.5) + 0.8)*(#7)}
  \let\pgfpie@innerpos\pgfmathresult

  \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{%
    % label and number together
    \path (pgfpie@O) -- ++({\pgfpie@midangle}:{\pgfpie@innerpos}) node[align=center]
    {\pgfpie@scalefont{#3}\pgfpie@labeltext{#4}\\\pgfpie@numbertext{#3}};
  }{%
    % label
    \pgfpie@ifhidelabel{}{%
      \pgfpie@iflegend{}{%
        \path (pgfpie@O) -- ++ ({\pgfpie@midangle}:{\pgfpie@radius})
        node[inner sep=0, \pgfpie@text={\pgfpie@midangle:#4}]{};
      }%
    }%

    % number
    \path (pgfpie@O) -- ++({\pgfpie@midangle}:{\pgfpie@innerpos}) node
    {\pgfpie@scalefont{#3}\pgfpie@numbertext{#3}};
  }%
}

\def\pgfpie@findColor#1{%
  \pgfmathparse{int(mod(#1,\the\pgfpie@colorLength))}%
  \let\pgfpie@ci\pgfmathresult
  \foreach \pgfpie@c [count=\pgfpie@j from 0] in \pgfpie@color {%
    \pgfpie@ifnum{\pgfpie@j}{=}{\pgfpie@ci}{%
      \xdef\pgfpie@thecolor{\pgfpie@c}%
      \breakforeach
    }{}%
  }
}

\def\pgfpie@findExplode#1{%
  \pgfmathparse{int(mod(#1,\the\pgfpie@explodeLength))}%
  \let\pgfpie@ei\pgfmathresult
  \foreach \pgfpie@e [count=\pgfpie@j from 0] in \pgfpie@explode {%
    \pgfpie@ifnum{\pgfpie@j}{=}{\pgfpie@ei}{%
      \xdef\pgfpie@theexplode{\pgfpie@e}%
      \breakforeach
    }{}%
  }%
}

% #1: bottom left point
% #2: size
% #3: number
% #4: color
% #5: text
\def\pgfpie@square#1#2#3#4#5{%
  \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{%
    \draw[fill={#4},\pgfpie@style] (#1) rectangle node[align=center]
    {\pgfpie@scalefont{#3}\pgfpie@labeltext{#5}\\\pgfpie@numbertext{#3}} ++(#2);
  }{%
    \draw[fill={#4},\pgfpie@style] (#1) rectangle node
    {\pgfpie@scalefont{#3}\pgfpie@numbertext{#3}} ++(#2);
  }%
}

% #1: pos
% #2: radius
% #3: number
% #4: color
% $5: style
% $6: label
\def\pgfpie@cloud#1#2#3#4#5#6{%
  \draw[fill=#4, #5] (#1) circle[radius=#2];
  \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{%
    \node[align=center] at (#1) {\pgfpie@scalefont{#3}\pgfpie@labeltext{#6}\\\pgfpie@numbertext{#3}};
  }{%
    \node at (#1) {\pgfpie@scalefont{#3}\pgfpie@numbertext{#3}};
  }%
}

\newdimen\pgfpie@angleEnd
\newcount\pgfpie@explodeLength
\newcount\pgfpie@colorLength
\newcount\pgfpie@sliceLength

\pgfqkeys{/pgfpie}{%
  .search also={/tikz,/pgf},
  explode/.store in=\pgfpie@explode,
  color/.store in=\pgfpie@color,
  radius/.store in=\pgfpie@radius,
  pos/.store in=\pgfpie@pos,
  style/.store in=\pgfpie@style,
  before number/.store in=\pgfpie@beforenumber,
  after number/.code={%
    \def\pgfpie@afternumber{#1}%
    \def\pgfpie@late@afternumber{}%
  },
  text/.store in=\pgfpie@text,
  sum/.code={%
    \def\pgfpie@sum{#1}%
    \pgfpie@ifx\pgfpie@sum\pgfpie@sum@c{%
      \def\pgfpie@late@afternumber{\def\pgfpie@afternumber{\%}}%
    }{%
      \def\pgfpie@late@afternumber{}%
    }%
  },
  rotate/.store in=\pgfpie@rotate,
}

\pgfpie@newif{polar}
\pgfqkeys{/pgfpie}{polar/.is if=pgfpie@polar}

\pgfpie@newif{legend}

\pgfpie@newif{changedirection}
\pgfqkeys{/pgfpie}{change direction/.is if=pgfpie@changedirection}

\pgfpie@newif{square}
\pgfqkeys{/pgfpie}{square/.is if=pgfpie@square}

\pgfpie@newif{cloud}
\pgfqkeys{/pgfpie}{cloud/.is if=pgfpie@cloud}

\pgfpie@newif{scalefont}
\pgfqkeys{/pgfpie}{scale font/.is if=pgfpie@scalefont}
\def\pgfpie@scalefont#1{%
  \pgfpie@ifscalefont{%
    \pgfmathparse{(#1) / (\pgfpie@sum) * 3 + 0.9}%
    \scalefont{\pgfmathresult}%
  }{}%
}

\pgfpie@newif{hidenumber}
\pgfqkeys{/pgfpie}{hide number/.is if=pgfpie@hidenumber}
\def\pgfpie@numbertext#1{%
  \pgfpie@ifhidenumber{}{%
    \pgfpie@beforenumber#1\pgfpie@afternumber
  }%
}

\pgfpie@newif{hidelabel}
\pgfqkeys{/pgfpie}{hide label/.is if=pgfpie@hidelabel}
\def\pgfpie@labeltext#1{\pgfpie@ifhidelabel{}{#1}}

\tikzaddtikzonlycommandshortcutlet{\pie}{\pgfpie@pie}%

\def\pgfpie@pie{%
  \pgfutil@ifnextchar[{\pgfpie@@pie}{\pgfpie@@pie[]}%
}

\def\pgfpie@@pie[#1]#2{%
  \scope[%
    % to be compatible with "babel" lib
    handle active characters in nodes=false,
    % load default parameters
    /pgfpie/.cd,
    explode=0,
    color={blue!60, cyan!60, yellow!60, orange!60, red!60,
      blue!60!cyan!60, cyan!60!yellow!60, red!60!cyan!60,
      red!60!blue!60, orange!60!cyan!60},
    radius=3,
    pos={0,0},
    style={thick},
    before number=,
    after number=,
    text=label,
    sum=100,
    rotate=0,
    change direction=false,
    polar=false,
    square=false,
    cloud=false,
    scale font=false,
    hide number=false,
    hide label=false,
    every pie/.try,%
    % load user's parameters
    #1]

  % add percentage automatically
  \pgfpie@late@afternumber

  % legend or not
  \pgfpie@ifx\pgfpie@text\pgfpie@text@legend{%
    \pgfpie@legendtrue
  }{%
    \pgfpie@legendfalse
  }%

  % handle sum
  \pgfpie@ifx\pgfpie@sum\pgfpie@sum@auto{%
    % sum all input
    \xdef\pgfpie@sum{0}%
    \foreach \pgfpie@p/\pgfpie@t in {#2} {%
      \pgfmathparse{(\pgfpie@sum) + (\pgfpie@p)}%
      \xdef\pgfpie@sum{\pgfmathresult}%
    }%
  }{}%

  % init counters
  \global\pgfpie@explodeLength=0
  \foreach \pgfpie@e in \pgfpie@explode {%
    \global\advance\pgfpie@explodeLength by 1
  }%

  \global\pgfpie@colorLength=0
  \foreach \pgfpie@c in \pgfpie@color {%
    \global\advance\pgfpie@colorLength by 1
  }%
  
  \pgfmathsetlength{\pgfpie@angleEnd}{0}%

  \global\pgfpie@sliceLength=0
  \foreach \pgfpie@p/\pgfpie@e in {#2} {%
    \global\advance\pgfpie@sliceLength by 1
  }%

  \pgfpie@ifsquare{%
    \pgfpie@pie@square{#2}%
    }{\pgfpie@ifcloud{\pgfpie@pie@cloud{#2}%
      }{\pgfpie@pie@circle{#2}}}

  % legend
  \pgfpie@ifhidelabel{}{%
    \pgfpie@iflegend{%
      \pgfpie@legend{#2}%
  }{}}%
  \endscope
}

\def\pgfpie@pie@square#1{%
  \pgfmathparse{(\pgfpie@radius)*2}
  \xdef\pgfpie@verticalLength{\pgfmathresult}
  \xdef\pgfpie@horizontalLength{\pgfmathresult}
  \path (\pgfpie@pos) -- ++({-\pgfpie@radius},{-\pgfpie@radius}) coordinate (pgfpie@start);
  \pgfmathparse{(\pgfpie@verticalLength) * (\pgfpie@horizontalLength) / (\pgfpie@sum)}
  \let\pgfpie@squareUnit\pgfmathresult

  % drawing loop
  \foreach \pgfpie@p/\pgfpie@t [count=\pgfpie@i from 0] in {#1}
  {
    \pgfpie@findColor{\pgfpie@i}

    \pgfpie@ifdim{\pgfpie@verticalLength cm}{>}{\pgfpie@horizontalLength cm}{%
      \pgfmathparse{(\pgfpie@p) * (\pgfpie@squareUnit) / (\pgfpie@horizontalLength)}
      \let\pgfpie@height\pgfmathresult
      
      \pgfpie@square{pgfpie@start}{\pgfpie@horizontalLength,\pgfpie@height}
      {\pgfpie@p}
      {\pgfpie@thecolor}
      {\pgfpie@t}
      %label
      \pgfpie@iflegend{}{%
        \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{}{%
          \pgfpie@ifhidelabel{}{%
            \path (pgfpie@start) -- ++({\pgfpie@horizontalLength},{\pgfpie@height*0.5})
            node[inner sep=0, \pgfpie@text={0:{\pgfpie@t}}]{};
          }%
        }%
      }%

      \pgfmathparse{\pgfpie@verticalLength - \pgfpie@height}
      \xdef\pgfpie@verticalLength{\pgfmathresult}
      \path (pgfpie@start) -- ++(0, \pgfpie@height) coordinate (pgfpie@start);
    }{%
      \pgfmathparse{(\pgfpie@p) * (\pgfpie@squareUnit) / (\pgfpie@verticalLength)}%
      \let\pgfpie@width\pgfmathresult

      \pgfpie@square{pgfpie@start}{\pgfpie@width,\pgfpie@verticalLength}
      {\pgfpie@p}
      {\pgfpie@thecolor}
      {\pgfpie@t}
      %label
      \pgfpie@iflegend{}{%
        \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{}{%
          \pgfpie@ifhidelabel{}{%
            \path (pgfpie@start) -- ++({\pgfpie@width*0.5},{\pgfpie@verticalLength})
            node[inner sep=0, \pgfpie@text={90:{\pgfpie@t}}]{};
          }%
        }%
      }%

      \pgfmathparse{(\pgfpie@horizontalLength) - (\pgfpie@width)}%
      \xdef\pgfpie@horizontalLength{\pgfmathresult}%
      \path (pgfpie@start) -- ++({\pgfpie@width},0) coordinate (pgfpie@start);
    }%
  }%
}

\def\pgfpie@pie@cloud#1{%
  % drawing loop
  \foreach \pgfpie@p/\pgfpie@t [count=\pgfpie@i from 0] in {#1}
  {
    % find explode
    \pgfpie@findExplode{\pgfpie@i}
    \def\pgfpie@cloudGap{(\pgfpie@theexplode) + 0.1}
    \pgfmathparse{sqrt((\pgfpie@p) / (\pgfpie@sum)) * (\pgfpie@radius)}
    \let\pgfpie@cloudR\pgfmathresult
    \pgfpie@ifnum{\pgfpie@i}{=}{0}{%
      % first cloud
      \coordinate (pgfpie@O) at (\pgfpie@pos);
      \xdef\pgfpie@cloudRone{\pgfpie@cloudR}
      \xdef\pgfpie@cloudExtendDir{180+(\pgfpie@rotate)}
    }{\pgfpie@ifnum{\pgfpie@i}{=}{1}{%
      % second cloud
      \xdef\pgfpie@cloudRtwo{\pgfpie@cloudR}
      \xdef\pgfpie@cloudExtendDir{45+(\pgfpie@rotate)}
      \path (pgfpie@O) -- ++({\pgfpie@cloudExtendDir}:{(\pgfpie@cloudRone)+(\pgfpie@cloudGap)+(\pgfpie@cloudRtwo)}) coordinate (pgfpie@O);
    }{%
      % next cloud
      \pgfmathparse{(\pgfpie@cloudRone)+(\pgfpie@cloudGap)+(\pgfpie@cloudRtwo)}
      \let\pgfpie@la\pgfmathresult
      \pgfmathparse{(\pgfpie@cloudRone)+(\pgfpie@cloudGap)+(\pgfpie@cloudR)}
      \let\pgfpie@lb\pgfmathresult
      \pgfmathparse{(\pgfpie@cloudRtwo)+(\pgfpie@cloudGap)+(\pgfpie@cloudR)}
      \let\pgfpie@lc\pgfmathresult
      \pgfmathparse{(\pgfpie@la)^2+(\pgfpie@lc)^2-(\pgfpie@lb)^2}
      \let\pgfpie@tmp\pgfmathresult
      \pgfmathparse{180 - acos((\pgfpie@tmp) / 2 / (\pgfpie@la) / (\pgfpie@lc))}
      \let\pgfpie@cloudRot\pgfmathresult
      \pgfpie@ifodd{\pgfpie@i}{%
        \pgfmathparse{-(\pgfpie@cloudRot)}
        \let\pgfpie@cloudRot\pgfmathresult
      }{}%
      \pgfmathparse{(\pgfpie@cloudExtendDir) - (\pgfpie@cloudRot)}
      \xdef\pgfpie@cloudExtendDir{\pgfmathresult}
      \path (pgfpie@O) -- ++({\pgfpie@cloudExtendDir}:{\pgfpie@lc}) coordinate (pgfpie@O);
      \xdef\pgfpie@cloudRone{\pgfpie@cloudRtwo}
      \xdef\pgfpie@cloudRtwo{\pgfpie@cloudR}
    }}%

    % find color
    \pgfpie@findColor{\pgfpie@i}

    \pgfpie@cloud{pgfpie@O}{\pgfpie@cloudR}{\pgfpie@p}
    {\pgfpie@thecolor}{\pgfpie@style}{\pgfpie@t}

    % label
    \pgfpie@iflegend{}{%
      \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{}{%
        \pgfpie@ifhidelabel{}{%
          \path (pgfpie@O) -- ++({\pgfpie@cloudExtendDir}:{\pgfpie@cloudR})
          node[inner sep=0, \pgfpie@text={\pgfpie@cloudExtendDir:{\pgfpie@t}}] {};
        }%
      }%
    }%
  }%
}

\def\pgfpie@pie@circle#1{%
  \pgfpie@ifpolar{%
    \xdef\pgfpie@maxValue{0}
    \foreach \pgfpie@p/\pgfpie@e in {#1} {
      \pgfmathparse{\pgfpie@p}%
      \pgfpie@ifdim{\pgfpie@maxValue pt}{<}{\pgfmathresult pt}{%
        \xdef\pgfpie@maxValue{\pgfpie@p}
      }{}%
    }
    \pgfmathparse{(\pgfpie@sum) / \the\pgfpie@sliceLength}
    \xdef\pgfpie@polarangle{\pgfmathresult}
    \pgfmathparse{(\pgfpie@radius) / sqrt(\pgfpie@maxValue)}
    \xdef\pgfpie@polarRadiusUnit{\pgfmathresult}
  }{%
    \xdef\pgfpie@theradius{\pgfpie@radius}%
  }

  \pgfpie@ifchangedirection{%
    \pgfmathsetlength{\pgfpie@angleEnd}{\pgfpie@sum}
  }{}%
  \xdef\pgfpie@angleBegin{\the\pgfpie@angleEnd}
  % drawing loop
  \foreach \pgfpie@p/\pgfpie@t [count=\pgfpie@i from 0] in {#1}
  {
    \pgfmathsetlength{\pgfpie@angleEnd}{\pgfpie@angleBegin}
    \pgfpie@ifpolar{%
      % Polar area diagram
      \pgfmathaddtolength{\pgfpie@angleEnd}{\pgfpie@polarangle}
      \pgfmathparse{sqrt(\pgfpie@p) * (\pgfpie@polarRadiusUnit)}
      \xdef\pgfpie@theradius{\pgfmathresult}
    }{%
      % normal pie
      \pgfpie@ifchangedirection{%
        \pgfmathaddtolength{\pgfpie@angleEnd}{-(\pgfpie@p)}
      }{%
        \pgfmathaddtolength{\pgfpie@angleEnd}{\pgfpie@p}
      }%
    }%

    % find explode
    \pgfpie@findExplode{\pgfpie@i}

    % find color
    \pgfpie@findColor{\pgfpie@i}
    \pgfpie@slice{(\pgfpie@angleBegin)/(\pgfpie@sum)*360+(\pgfpie@rotate)}
    {\the\pgfpie@angleEnd/(\pgfpie@sum)*360+(\pgfpie@rotate)}
    {\pgfpie@p}
    {\pgfpie@t}
    {\pgfpie@theexplode}
    {\pgfpie@thecolor}
    {\pgfpie@theradius}
    {\pgfpie@pos}
    \xdef\pgfpie@angleBegin{\the\pgfpie@angleEnd}
  }
}

\def\pgfpie@legend#1{%
  \coordinate[xshift=0.8cm,
  yshift={(\the\pgfpie@sliceLength*0.5+1)*0.5cm}] (pgfpie@legendpos) at
  (current bounding box.east);

  \scope[node distance=0.5cm]
    \foreach \pgfpie@p/\pgfpie@t [count=\pgfpie@i from 0] in {#1}
    {
      \pgfpie@findColor{\pgfpie@i}
      \node[draw, fill={\pgfpie@thecolor}, \pgfpie@style, below of={pgfpie@legendpos}, label={0:{\pgfpie@t}}] (pgfpie@legendpos) {};
    }
  \endscope
}

